Challenger-Based Combinatorial Bandits for Subcarrier Selection in OFDM Systems

This paper investigates the identification of the top-m user-scheduling sets in multi-user MIMO downlink, which is cast as a combinatorial pure-exploration problem in stochastic linear bandits. Because the action space grows exponentially, exhaustive search is infeasible. We therefore adopt a linear utility model to enable efficient exploration and reliable selection of promising user subsets. We introduce a gap-index framework that maintains a shortlist of current estimates of champion arms (top-m sets) and a rotating shortlist of challenger arms that pose the greatest threat to the champions. This design focuses on measurements that yield the most informative gap-index-based comparisons, resulting in significant reductions in runtime and computation compared to state-of-the-art linear bandit methods, with high identification accuracy. The method also exposes a tunable trade-off between speed and accuracy. Simulations on a realistic OFDM downlink show that shortlist-driven pure exploration makes online, measurement-efficient subcarrier selection practical for AI-enabled communication systems.

==> plots/K_40/comparisons_plot.tex <==
\begin{tikzpicture}

    \begin{axis}[
        ybar=0.2pt,
            width=4cm,
            height=4.2cm,
            bar width=0.45,
            bar shift=0pt,
            every axis plot/.append style={fill},
            grid=major,
            xticklabel style={rotate=45},
            xtick={1, 2, 3},
            xticklabels={\name{}, LinGapE, LinGIFA},
            xlabel={},
            ylabel style = {font= \tiny},
        yticklabel style = {font=\boldmath \tiny, xshift=0.2ex},
        xticklabel style ={font=\small , yshift=0.2ex},
            ylabel={Avg no. of comparisons (in $10^5$) },
            enlarge x limits=0.25,
            ymin=0,
            ymax=3900000,
            legend style ={font=\small,yshift=0.5ex},
            area legend,
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend pos=north west,
            legend columns=-1,
            legend style={/tikz/every even column/.append style={column sep=0.2cm}},
        ]
        \addplot+[
            ybar=0.2pt,
            plotColor1*,
            draw=black,
            error bars/.cd,
                y dir=both,
                y explicit,
        ] plot coordinates {
                (1,0.564914) +- (0,0.008676)
            };
            \addplot+[           ybar,
            plotColor2*,
            draw=black,
            postaction={
                    pattern=north east lines
                },
            error bars/.cd,
                y dir=both,
                y explicit,] plot coordinates {           
                (2,32866.658348) +- (0,2080.473126)
                };

                        \addplot+[
            ybar,
            plotColor4*,
            draw=black,
            postaction={
                    pattern=north east lines
                },
            error bars/.cd,
                y dir=both,
                y explicit,
        ] plot coordinates {
              (3,3292288.6) +- (0,752860.94)
            };

 

    \end{axis}
\end{tikzpicture}

